QuantaAlpha: An Evolutionary Framework for LLM-Driven Alpha Mining

Financial markets are noisy and non-stationary, making alpha mining highly sensitive to backtest noise and regime shifts. While recent agentic frameworks improve automation, they often lack controllable multi-round search and reliable reuse of validated experience. To address these challenges, we propose QuantaAlpha, an evolutionary alpha mining framework that treats each end-to-end mining run as a trajectory and improves factors via trajectory-level mutation and crossover. QuantaAlpha localizes suboptimal steps for targeted revision and recombines complementary high-reward segments to reuse effective patterns, enabling structured exploration and refinement across iterations. During factor generation, it enforces semantic consistency across hypothesis, factor expression, and executable code, and constrains the complexity and redundancy of the generated factor to mitigate crowding. Extensive experiments on CSI 300 show consistent gains over strong baselines and prior agentic systems. Using GPT-5.2, QuantaAlpha achieves an IC of 0.0472 with ARR of 4.68% and MDD of 11.8%. Moreover, factors mined on CSI 300 transfer effectively to CSI 500 and the S&P 500, delivering about 40.28% and 19.1% cumulative excess return over four years, respectively, which indicates strong robustness under market distribution shifts.

==> main_section/3.problem_formulation_backup.tex <==
\section{Problem Formulation}
The goal of alpha mining is to automatically construct a set of computable functions that map historical market data to predictive signals. Given a stock universe $U = \{s_1, \dots, s_N\}$ and a set of trading days $T = \{t_1, \dots, t_M\}$, for any stock $i \in U$ at time $t \in T$, let $X_{\le t, i}$ denote the historical observation sequence (e.g., OHLC). An alpha factor is defined as a scoring function $f: \mathcal{X} \to \mathbb{R}$ within a symbolic expression space $\mathcal{F}$ induced by a Domain-Specific Language (DSL):
\begin{equation}
    \text{score}(t, i) = f(X_{\le t, i}), \quad f \in \mathcal{F}
    \label{eq:alpha_def}
\end{equation}
These scores are used to predict future returns, supporting cross-sectional ranking or portfolio construction.

We formulate alpha mining as a black-box search problem over $\mathcal{F}$. Let $y$ denote the ground-truth forward returns serving as prediction targets (e.g., $y_{t,i} = r_{t+1,i}$ for next-day returns). Under a fixed backtesting protocol $B$, each candidate factor $f$ is evaluated against $(X, y)$ to yield a vector of performance metrics:
\begin{equation}
    m(f)=\mathrm{Eval}\!\left(f;\,X,y,B\right)\in\mathbb{R}^{K},
    \label{eq:metric_vec}
\end{equation}
where $m(f)$ includes metrics such as IC, ARR, and risk-related measures. To facilitate optimization, this vector is further mapped to a scalar objective $u(f) = \phi(\mathbf{m}(f))$ for ranking and selection. 

However, the ultimate goal is not merely to identify a single valid factor, but to construct a diverse and reusable factor library $P \subset \mathcal{F}$. Therefore, we pose the library construction as a subset selection problem to maximize a collective objective:
\begin{equation}
P^* = \arg \max_{P \subset \mathcal{F}} J(P),
\label{eq:global_obj}
\end{equation}
where $J(P)$ measures the library-level utility of $P$, encouraging strong individual factors while promoting diversity and complementarity within the set. 



==> main_section/4.method_backup.tex <==
\section{Method}

To automate the discovery of high-quality alpha factors, we propose \method, a \textit{coarse-to-fine evolutionary framework} that bridges abstract financial intuition and executable factor expressions. We organize the mining process as a hierarchical cascade that separates the discovery of trading mechanisms from their executable realization, enabling structured exploration that is both broad in scope and precise in execution.

As illustrated in Figure~\ref{fig:framework.pdf}, our procedure consists of two collaborative stages. First, the Automated Hypothesis Discovery stage (Section~\ref{sec:4.1}) operates in the semantic space: it starts with Diversified Planning to establish broad initial coverage, and then applies a Self-Evolutionary Mechanism to maintain and refine a set of high-potential hypotheses. Second, these hypotheses are fed into the Controllable Factor Synthesis stage (Section~\ref{sec:4.2}), which generates executable factor expressions under strict feasibility constraints and feedback-driven refinement. 

Unlike prior approaches \cite{li2025rdagent, Tang2025AlphaAgent} that repeatedly revise individual candidates based on backtesting feedback—often overfitting to noise and inducing semantic drift—our framework adopts a self-evolutionary strategy at the hypothesis level. We evolve the hypotheses themselves so that each update produces a new, logically coherent financial proposition. Crucially, we use feedback in a fundamentally different way: instead of treating backtesting outcomes as a corrective signal to ``patch'' the current hypothesis, we use them strictly as a selection criterion. Backtesting evidence is only used to identify validated mechanisms from high-performing ancestors; these mechanisms are preserved as inheritable ``genes'' that guide subsequent hypothesis evolution. This evolutionary generative paradigm guarantees that the exploration remains controllable, while establishing a trustworthy lineage grounded in verified economic intuition.

\subsection{Automated Hypothesis Discovery}
\label{sec:4.1}
The goal of Automated Hypothesis Discovery is to maintain a continuously evolving set of market hypotheses that capture diverse, interpretable trading rationales. Rather than directly manipulating factor expressions, this stage operates purely at the semantic level, where hypotheses specify what economic behavior to exploit, without committing to how it is implemented.

Formally, let $\mathcal{H}$ denote the hypothesis space, where each $h \in \mathcal{H}$ represents a structured natural language description of a trading mechanism. The discovery process maintains a dynamic candidate set $H^r = \{h_1, \dots, h_n\} \subset \mathcal{H}$ at iteration $r$, evolving it to explore the semantic manifold efficiently.  

\subsubsection{Diversified Planning Initialization}
Since the hypothesis space is discrete and high-dimensional, and downstream evaluation relies on computationally expensive backtesting, the efficiency of the search is critically dependent on the coverage of the initial candidate set. A lack of diversity in the initialization $\mathcal{H}^0$ often confines subsequent evolution to a narrow local neighborhood, hindering global exploration.

To address this, we employ a diversified planning strategy to construct a structurally complementary initial set $H^0$ conditioned on a broad research direction $d$. We formulate this as:
\begin{equation}
H^0 = \text{Planner}(d, n) = \{h_1^0, \dots, h_n^0\},
\end{equation}
where $n$ controls the breadth of initial exploration. 

\subsubsection{Self-Evolution}

Once the initial set $H^0$ is established, the search process enters an iterative evolutionary cycle to expand the discovery frontier. Specifically, at each iteration $r$, we execute two operations based on the previous hypothesis set $H^{r-1}$: the mutation operator produces a mutation set $M^r$, and the crossover operator synthesizes a crossover set $C^r$. The hypothesis set for the current iteration is then formally constructed as the union of these two outcomes:
\begin{equation}
H^r = M^r \cup C^r.
\end{equation}

\paragraph{Orthogonal Mutation.} The primary objective of this operator is to continuously generate hypotheses that are mechanistically distinct from the existing set. By facilitating an extrapolative exploration of the hypothesis space, it expands the search frontier and mitigates the risk of local convergence. In essence, orthogonal mutation introduces novel mechanistic interpretations, thereby enhancing both the scope and diversity of the discovery process.

To realize this, the operator applies structural perturbations directly to the hypotheses resulting from the previous generation step. Specifically, the input source is the initial set $H^0$ for the first round ($r=1$) and the crossover set $C^{r-1}$ for all subsequent rounds ($r > 1$). Through this process, we derive the mutation set $M^r$.

Formally, for each hypothesis $h$ in the source set, the operator yields a variant
\begin{equation}
h' = \text{Mutate}(h).
\end{equation}
Crucially, we define this process as ``orthogonal'' because it enforces fundamental structural shifts rather than trivial semantic paraphrasing. By altering underlying mechanisms such as triggering conditions, data sources, or time scales, the operator compels the hypotheses to diverge into entirely distinct construction paths.

\paragraph{Compositional Crossover.} While mutation focuses on expanding the search frontier, the crossover operator emphasizes mechanism fusion by recombining validated elements from multiple parent hypotheses. In each iteration $r$, the operator selects $k$ parents from an elite pool $E^{r}$ to synthesize a new hypothesis:
\begin{equation}
h' = \text{Crossover}(h^{p1}, \dots, h^{pk}), \quad h^{pi} \in E^{r}.
\end{equation}
The elite pool $E^r$ is constructed by evaluating and ranking the union of the previous crossover set $C^{r-1}$ and the current mutation set $M^r$. Specifically, the quality of a hypothesis $h$ is determined by the collective backtesting utility of its generated factor set $S_{h,r}$, with the detailed protocols for factor generation and evaluation provided in Section~\ref{sec:4.2}.

The primary advantage of this operator lies in its ability to structurally integrate validated critical elements from high-performance parents. This synthesis yields complex hybrid mechanisms that are typically inaccessible through single-step mutations. Furthermore, this approach significantly enhances the reliability of the generated candidates. By constructing new hypotheses upon empirically verified foundations rather than random initialization, the crossover operator ensures that the search is anchored in high-confidence regions of the solution space, thereby increasing the probability of identifying robust factor families.


\subsection{Controllable Factor Synthesis}
\label{sec:4.2}
Given a market hypothesis $h$ derived from the discovery stage, the objective of this phase is to synthesize a corresponding set of executable factors $S_h$ that implement the abstract economic intuition. In this framework, the efficacy of the hypothesis $h$ is quantified by the collective performance of this derived set, providing the essential basis for selection in the evolutionary search. Simultaneously, valid factors within $S_h$ are archived into the final factor library $\mathcal{P}$.

\subsubsection{Hypothesis-Driven Factor Generation}
To operationalize the generation process, a robust mechanism is required to align executable logic with domain hypotheses. However, direct code generation faces significant operational barriers, including syntax instability, library version conflicts, and semantic drift in complex implementations. These challenges create a fundamental tension between code executability and semantic consistency. To address these limitations, we introduce a standardized Operator Library $\mathcal{O}$ that abstracts mathematical and financial primitives (e.g., \texttt{TS\_MIN($\cdot$)}, \texttt{SMA($\cdot$)}, \texttt{RANK($\cdot$)}) into a consistent functional set. This abstraction layer bridges the gap between high-level market insights and low-level implementation details, forming the foundational vocabulary for our structured search space.

Building upon this standardized library, we adopt a progressive instantiation paradigm that transforms abstract hypotheses into executable code through a strictly controlled pipeline. We formally define this synthesis as a mapping $G: \mathcal{H} \times \mathcal{X} \to \mathcal{F}$, where $\mathcal{H}$ represents the hypothesis space, $\mathcal{X}$ denotes the raw feature space, and $\mathcal{F}$ contains tree-structured factors formed by symbolic assembly. The parsing procedure unfolds in three deterministic steps:

\textbf{(1) Semantic Mapping ($h \to des$):} The system first translates the textual hypothesis $h$ into a structured Semantic Description $des$. In this step, key phrases in $h$ (e.g., ``breakout pattern'', ``volatility contraction'') are identified and mapped to functional intents within the Operator Library $\mathcal{O}$, while numeric parameters (e.g., window size, threshold) are assigned based on explicit constraints or domain-adaptive defaults.

\textbf{(2) Symbolic Assembly ($des \to f$):} Conditioned on the description $des$, the system synthesizes the concrete symbolic expression $f$ and parses it into an Abstract Syntax Tree (AST), denoted as $T(f)$. This structure captures the computational dependencies and execution flow. In $T(f)$, leaf nodes correspond to raw feature references (e.g., \texttt{\$high}, \texttt{\$volume}), while internal nodes represent operator instances that transform the data stream.

\textbf{(3) Deterministic Compilation ($f \to c$):} Finally, distinct from stochastic code generation, the validated AST is mechanically translated into executable code $c$. This ensures that the final implementation is strictly isomorphic to the symbolic definition $f$, eliminating the risk of syntax errors or logic hallucinations.

By structuring the generation process, we guarantee that every synthesized factor is rooted in a clear economic intent and realized through a verifiable computational structure.

% via Feedback
\subsubsection{Complexity and Redundancy Control}




\subsubsection{Backtesting}

==> tables/2.app_2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Color definitions for tcolorbox
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{headerblue}{RGB}{41, 128, 185}
\definecolor{metricgreen}{RGB}{39, 174, 96}
\definecolor{alertred}{RGB}{192, 57, 43}
\definecolor{warningyellow}{RGB}{243, 156, 18}
\definecolor{lightgray}{RGB}{245, 245, 245}
\definecolor{darkgray}{RGB}{52, 73, 94}
\definecolor{mutationpurple}{RGB}{142, 68, 173}
\definecolor{crossoverblue}{RGB}{52, 152, 219}

% tcolorbox library
\tcbuselibrary{skins,breakable}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Case Study: Factor Evolution Trajectory}
\label{sec:appendix_case_study}

This appendix presents a detailed case study of factor evolution in QuantaAlpha. We trace the complete trajectory of a representative factor---\textit{Institutional\_Momentum\_Score\_20D}---through the crossover phase, demonstrating how the evolutionary framework synthesizes complementary market hypotheses from parent trajectories.

QuantaAlpha's evolution process operates in three phases: (1) \textbf{Original} phase where initial hypotheses are generated, (2) \textbf{Mutation} phase where existing trajectories are perturbed to explore diversified strategies, and (3) \textbf{Crossover} phase where high-performing parent trajectories are combined to synthesize offspring with potentially superior predictive power. The following factor card illustrates a Round 8 Crossover operation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Factor Identity Card
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Factor Identity}

The factor card below presents the basic information of the evolved factor, including its unique identifiers, evolution lineage, and mathematical formulation.

\begin{tcolorbox}[
  colback=lightgray,
  colframe=headerblue,
  fonttitle=\bfseries\large,
  title={\faTag\ Institutional\_Momentum\_Score\_20D},
  arc=3mm,
  boxrule=1pt
]

\begin{tabular}{@{}ll@{}}
\textbf{Factor ID:} & \texttt{c57cace576a95356} \\
\textbf{Trajectory ID:} & \texttt{df5a496878f4} \\
\textbf{Evolution Round:} & Round 8 \\
\textbf{Evolution Phase:} & \colorbox{crossoverblue!20}{\textcolor{crossoverblue}{\textbf{Crossover}}} \\
\textbf{Direction ID:} & 6 \\
\end{tabular}

\vspace{0.3cm}

\textbf{Factor Expression:}
\begin{tcolorbox}[colback=darkgray!5, colframe=darkgray, boxrule=0.3pt, arc=1mm]
\small\ttfamily
RANK(TS\_CORR(DELTA(\$close, 1)/\$close, DELTA(\$volume, 1)/\$volume, 20) * TS\_MEAN((\$close - \$open)/\$close, 5))
\end{tcolorbox}

\textbf{Mathematical Formulation:}
\[
\text{IMS}_{20D} = \text{RANK}\left(\rho_{20}\left(\frac{\Delta P}{P}, \frac{\Delta V}{V}\right) \times \overline{\left(\frac{C - O}{C}\right)}_{5}\right)
\]

where $\rho_{20}(\cdot,\cdot)$ denotes the 20-day rolling correlation, $\Delta P/P$ is the daily return, $\Delta V/V$ is the volume change ratio, and $\overline{(\cdot)}_5$ is the 5-day moving average.

\vspace{0.2cm}

\textbf{Factor Interpretation:}\\
\small
This factor captures institutional-driven momentum by measuring two key signals: (1) the correlation between price returns and volume changes, which indicates coordinated institutional trading when positive; and (2) the average intraday return pattern, reflecting institutional activity that typically influences closing prices. The cross-sectional ranking ensures comparability across stocks.

\end{tcolorbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Evolution Lineage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evolution Lineage}

The crossover operation combines insights from two parent trajectories with complementary market hypotheses. Parent 1 focuses on identifying \textit{fragile momentum} driven by retail speculation, while Parent 2 targets \textit{sustainable momentum} supported by institutional activity. The LLM synthesizes these complementary perspectives into a unified framework.

\begin{tcolorbox}[
  colback=purple!5,
  colframe=mutationpurple,
  fonttitle=\bfseries,
  title={\faDna\ Evolution Information},
  arc=2mm,
  boxrule=0.5pt
]

\textbf{\faCodeBranch\ Parent Trajectories:}

\vspace{0.3cm}

\begin{minipage}[t]{0.48\textwidth}
\begin{tcolorbox}[colback=mutationpurple!5, colframe=mutationpurple!50, boxrule=0.3pt, title={\small\textbf{Parent 1: 1e6d57e38e89}}, fonttitle=\bfseries\small]
\small
\begin{tabular}{@{}ll@{}}
\textbf{Round:} & Round 7 \\
\textbf{Phase:} & Mutation \\
\textbf{Rank IC:} & 0.0216 \\
\textbf{IC:} & 0.0059 \\
\textbf{IR:} & 1.297 \\
\end{tabular}

\vspace{0.2cm}
\textbf{Core Hypothesis:}\\
\scriptsize When retail investors exhibit herd behavior and momentum chasing in stocks with high social media activity, but accompanied by declining institutional ownership and deteriorating fundamentals, the resulting price momentum is unsustainable and leads to mean reversion.
\end{tcolorbox}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\begin{tcolorbox}[colback=crossoverblue!5, colframe=crossoverblue!50, boxrule=0.3pt, title={\small\textbf{Parent 2: 47e0f0e55382}}, fonttitle=\bfseries\small]
\small
\begin{tabular}{@{}ll@{}}
\textbf{Round:} & Round 6 \\
\textbf{Phase:} & Crossover \\
\textbf{Rank IC:} & 0.0246 \\
\textbf{IC:} & 0.0069 \\
\textbf{IR:} & 1.347 \\
\end{tabular}

\vspace{0.2cm}
\textbf{Core Hypothesis:}\\
\scriptsize A regime-adaptive structural momentum factor combining institutional ownership-driven medium-term price trends with short-term microstructure regime validation, where coordinated accumulation/distribution patterns amplify momentum when confirmed by microstructure alignment.
\end{tcolorbox}
\end{minipage}

\vspace{0.3cm}

\textbf{\faSitemap\ Evolution Path Diagram:}
\begin{center}
\begin{tikzpicture}[
    node distance=2cm,
    roundbox/.style={rectangle, rounded corners, draw=headerblue, fill=headerblue!10, minimum width=3cm, minimum height=1cm, align=center, font=\small},
    arrow/.style={->, thick, >=stealth}
]
    % Parent nodes
    \node[roundbox, fill=mutationpurple!10, draw=mutationpurple] (p1) at (-3, 2) {Parent 1\\Round 7 Mutation\\Rank IC: 0.0216};
    \node[roundbox, fill=crossoverblue!10, draw=crossoverblue] (p2) at (3, 2) {Parent 2\\Round 6 Crossover\\Rank IC: 0.0246};
    
    % Current node
    \node[roundbox, fill=metricgreen!20, draw=metricgreen, minimum width=4cm] (current) at (0, 0) {\textbf{Offspring Factor}\\Round 8 Crossover\\Rank IC: \textbf{0.0311}};
    
    % Arrows
    \draw[arrow, mutationpurple] (p1) -- (current);
    \draw[arrow, crossoverblue] (p2) -- (current);
    
    % Label
    \node[font=\scriptsize\color{metricgreen}] at (0, -0.8) {$\uparrow$ 27\% improvement over best parent};
\end{tikzpicture}
\end{center}

\end{tcolorbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Synthesized Hypothesis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Synthesized Hypothesis}

Through crossover, the LLM generates a new hypothesis that integrates the complementary insights from both parents, rather than simply averaging their factor expressions. This hypothesis-driven approach ensures that the offspring factor captures genuinely novel market dynamics.

\begin{tcolorbox}[
  colback=blue!5,
  colframe=headerblue!70,
  fonttitle=\bfseries,
  title={\faLightbulb\ Hypothesis},
  arc=2mm,
  boxrule=0.5pt
]

\textbf{Core Hypothesis:}\\
A regime-aware dual-source momentum factor that combines institutional-driven structural momentum (validated by healthy microstructure) and retail-driven speculative momentum (characterized by high attention and deteriorating fundamentals), dynamically weighted by market volatility: amplifying institutional signals in stable regimes and retail reversal signals in turbulent regimes, will generate superior predictive returns.

\vspace{0.3cm}

\begin{tabular}{@{}p{0.28\textwidth}p{0.67\textwidth}@{}}
\toprule
\textbf{Component} & \textbf{Description} \\
\midrule
\textbf{Observation} & Parent strategies separately targeting institutional trends and retail herding show moderate predictive power (Rank IC $\sim$0.02--0.025), suggesting combined signals could capture complementary market dynamics. \\
\midrule
\textbf{Justification} & Sustainable price trends require institutional sponsorship and orderly trading, while retail-driven bubbles lack fundamental support and reverse under stress; a hybrid model exploiting both can enhance robustness across market regimes. \\
\midrule
\textbf{Domain Knowledge} & Institutional accumulation with strong price-volume correlation and low volatility indicates sustainable momentum; retail herding with declining institutional ownership and high volatility signals fragile momentum prone to reversal. \\
\bottomrule
\end{tabular}

\end{tcolorbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Backtest Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Backtest Performance}

After factor construction, QuantaAlpha automatically backtests the generated factors using the Qlib framework. The results below compare the offspring factor against both parent trajectories and the baseline, demonstrating the effectiveness of the crossover operation.

\begin{tcolorbox}[
  colback=green!5,
  colframe=metricgreen,
  fonttitle=\bfseries,
  title={\faChartLine\ Backtest Metrics},
  arc=2mm,
  boxrule=0.5pt
]

\begin{center}
\begin{tabular}{@{}lccc@{}}
\toprule
\textbf{Metric} & \textbf{Offspring Factor} & \textbf{Baseline} & \textbf{vs Baseline} \\
\midrule
\textbf{IC} & 0.0126 & 0.0058 & \textcolor{metricgreen}{$\uparrow$ 117\%} \\
\textbf{ICIR} & 0.0781 & -- & -- \\
\textbf{Rank IC} & \textbf{0.0311} & 0.0220 & \textcolor{metricgreen}{$\uparrow$ 41\%} \\
\textbf{Rank ICIR} & 0.1932 & -- & -- \\
\midrule
\textbf{ARR (Excess)} & 7.80\% & 5.20\% & \textcolor{metricgreen}{$\uparrow$ 50\%} \\
\textbf{IR} & 0.963 & 0.973 & \textcolor{alertred}{$\downarrow$ 1\%} \\
\textbf{MDD (Excess)} & $-$11.37\% & $-$7.30\% & \textcolor{alertred}{$\downarrow$ 56\%} \\
\bottomrule
\end{tabular}
\end{center}

\vspace{0.3cm}

\textbf{Detailed Statistics:}
\begin{center}
\small
\begin{tabular}{@{}ll|ll@{}}
\toprule
\textbf{Metric} & \textbf{Value} & \textbf{Metric} & \textbf{Value} \\
\midrule
Daily Excess Return (w/o cost) & 0.0328\% & Daily Excess Return (w/ cost) & 0.0128\% \\
Excess Return Std & 0.52\% & Turnover (FFR) & 100\% \\
L2 Train Loss & 0.9936 & L2 Valid Loss & 0.9962 \\
\bottomrule
\end{tabular}
\end{center}

\end{tcolorbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LLM Feedback
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{LLM Feedback and Iteration Guidance}

After evaluating backtest results, the LLM provides structured feedback that guides subsequent evolution rounds. This feedback loop enables continuous improvement by learning from both successes and failures.

\begin{tcolorbox}[
  colback=yellow!5,
  colframe=warningyellow,
  fonttitle=\bfseries,
  title={\faComments\ Feedback \& Evaluation},
  arc=2mm,
  boxrule=0.5pt
]

\textbf{\faSearch\ Observations:}\\
The crossover operation produced mixed results compared to the baseline:
\begin{itemize}
    \item \textcolor{metricgreen}{\faCheckCircle} Higher annualized excess return (7.80\% vs 5.20\%)
    \item \textcolor{metricgreen}{\faCheckCircle} Stronger IC (0.0126 vs 0.0058), indicating improved predictive power
    \item \textcolor{metricgreen}{\faCheckCircle} Rank IC improved 27\% over best parent (0.0311 vs 0.0246)
    \item \textcolor{alertred}{\faTimesCircle} Larger maximum drawdown ($-$11.37\% vs $-$7.30\%)
    \item \textcolor{alertred}{\faTimesCircle} Slightly lower information ratio (0.963 vs 0.973)
\end{itemize}

\vspace{0.2cm}

\textbf{\faBalanceScale\ Hypothesis Evaluation:}\\
Results partially support the hypothesis. Improved annualized return and IC suggest that combining institutional and retail momentum signals has merit. However, deterioration in risk metrics indicates that without proper regime-adaptive weighting, the combined signals may amplify risks during turbulent periods. The full hypothesis requires all three components (institutional momentum, retail herding reversal, volatility-adaptive weighting) to work effectively.

\vspace{0.2cm}

\textbf{\faFlag\ Decision:} \colorbox{alertred!20}{\textcolor{alertred}{\textbf{REJECTED}}} for direct deployment

\vspace{0.2cm}

\textbf{\faExclamationTriangle\ Recommendations for Next Iteration:}
\begin{enumerate}
    \item Use 20-day price-volume correlation as institutional momentum proxy
    \item Use 5-day average intraday returns as retail attention proxy
    \item Add volatility regime indicator (recent/historical volatility ratio) for dynamic weighting
\end{enumerate}

\small This feedback will inform the next mutation round, guiding the LLM to simplify the factor expression while preserving the core dual-source concept.

\end{tcolorbox}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Summary
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Key Takeaways}

This case study demonstrates several key aspects of QuantaAlpha's evolutionary factor mining:

\begin{enumerate}
    \item \textbf{Hypothesis-Driven Crossover}: The LLM synthesizes complementary market hypotheses rather than simply combining factor expressions, producing genuinely novel insights.
    
    \item \textbf{Measurable Improvement}: The offspring achieved 27\% Rank IC improvement over the best parent (0.0311 vs 0.0246), validating the crossover mechanism.
    
    \item \textbf{Return-Risk Trade-off}: While predictive power improved, risk metrics deteriorated, highlighting the importance of balanced optimization.
    
    \item \textbf{Structured Feedback}: Even rejected factors provide actionable guidance for subsequent iterations, enabling continuous improvement.
    
    \item \textbf{Interpretability}: Throughout evolution, factors remain interpretable via natural language hypotheses and mathematical formulations.
\end{enumerate}

This iterative process of hypothesis generation $\to$ factor construction $\to$ backtesting $\to$ feedback enables QuantaAlpha to systematically explore the factor space while maintaining interpretability and preventing overfitting.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/3.app_3.tex <==
\section{Case Study: Factor Evolution Trajectory}
\label{sec:appendix_case_study}

This appendix presents a detailed case study illustrating the factor evolution process in QuantaAlpha. We trace the complete trajectory of a representative factor---\textit{Institutional\_Momentum\_Score\_20D}---from its parent hypotheses through crossover recombination to its final form, demonstrating how the evolutionary framework synthesizes complementary market insights.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Overview of the Evolution Process}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

QuantaAlpha employs an evolutionary algorithm inspired by genetic programming, where factors evolve through three distinct phases:

\begin{enumerate}
    \item \textbf{Original Phase (Round 0)}: The LLM generates initial factor hypotheses across $N$ parallel exploration directions, creating the founding population of factor trajectories.
    
    \item \textbf{Mutation Phase (Odd Rounds)}: Existing trajectories undergo perturbation to explore diversified strategies, preventing convergence to local optima.
    
    \item \textbf{Crossover Phase (Even Rounds)}: High-performing parent trajectories are selected and combined, synthesizing their complementary strengths into offspring factors with potentially superior predictive power.
\end{enumerate}

The following case study demonstrates a \textbf{Crossover} operation at Round 8, where two parent trajectories with distinct market hypotheses are combined to create a regime-aware momentum factor.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Factor Identity Card}
\label{subsec:factor_card}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Table~\ref{tab:factor_identity} summarizes the basic information of the evolved factor.

\begin{table}[htbp]
\centering
\caption{Factor Identity Information}
\label{tab:factor_identity}
\begin{tabular}{ll}
\toprule
\textbf{Attribute} & \textbf{Value} \\
\midrule
Factor Name & Institutional\_Momentum\_Score\_20D \\
Factor ID & \texttt{c57cace576a95356} \\
Trajectory ID & \texttt{df5a496878f4} \\
Evolution Round & Round 8 \\
Evolution Phase & Crossover \\
Direction ID & 6 \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Factor Expression}

The final factor expression combines price-volume correlation with intraday return patterns:

\begin{equation}
\small
\texttt{RANK}\left(\texttt{TS\_CORR}\left(\frac{\Delta\texttt{close}}{\texttt{close}}, \frac{\Delta\texttt{volume}}{\texttt{volume}}, 20\right) \times \texttt{TS\_MEAN}\left(\frac{\texttt{close} - \texttt{open}}{\texttt{close}}, 5\right)\right)
\end{equation}

In mathematical notation:
\begin{equation}
\text{IMS}_{20D} = \text{RANK}\left(\rho_{20}\left(\frac{P_t - P_{t-1}}{P_{t-1}}, \frac{V_t - V_{t-1}}{V_{t-1}}\right) \times \frac{1}{5}\sum_{i=0}^{4}\frac{C_{t-i} - O_{t-i}}{C_{t-i}}\right)
\end{equation}

where $\rho_{20}(\cdot, \cdot)$ denotes the 20-day rolling Pearson correlation, $P_t$ is the closing price, $V_t$ is the trading volume, $C_t$ and $O_t$ are the close and open prices respectively.

\subsubsection{Factor Interpretation}

This factor captures \textbf{institutional-driven momentum signals} through two components:

\begin{itemize}
    \item \textbf{Price-Volume Correlation}: A positive correlation between returns and volume changes indicates coordinated institutional trading, where large players accumulate (distribute) positions with increasing volume during price advances (declines).
    
    \item \textbf{Intraday Return Pattern}: The average ratio of (close $-$ open) to close over 5 days reflects institutional activity patterns, as institutional traders often influence closing prices more than opening prices due to end-of-day portfolio adjustments.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evolution Lineage}
\label{subsec:evolution_lineage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The crossover operation combines insights from two parent trajectories with complementary market hypotheses. Table~\ref{tab:parent_trajectories} summarizes the parent information.

\begin{table}[htbp]
\centering
\caption{Parent Trajectory Information}
\label{tab:parent_trajectories}
\small
\begin{tabular}{lcc}
\toprule
\textbf{Attribute} & \textbf{Parent 1} & \textbf{Parent 2} \\
\midrule
Trajectory ID & \texttt{1e6d57e38e89} & \texttt{47e0f0e55382} \\
Evolution Round & Round 7 & Round 6 \\
Evolution Phase & Mutation & Crossover \\
\midrule
\multicolumn{3}{l}{\textit{Performance Metrics}} \\
IC & 0.0059 & 0.0069 \\
Rank IC & 0.0216 & 0.0246 \\
Information Ratio & 1.297 & 1.347 \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Parent 1: Retail Herding Hypothesis}

\textbf{Core Hypothesis}: \textit{``When retail investors exhibit herd behavior and momentum chasing in stocks with high social media activity and search volume, but accompanied by declining institutional ownership and deteriorating fundamental quality, the resulting price momentum is unsustainable and leads to significant mean reversion.''}

This parent trajectory focused on identifying \textbf{fragile momentum} driven by retail speculation, hypothesizing that such momentum lacks fundamental support and is prone to reversal.

\subsubsection{Parent 2: Institutional Momentum Hypothesis}

\textbf{Core Hypothesis}: \textit{``A regime-adaptive structural momentum factor combining institutional ownership-driven medium-term price trends with short-term microstructure regime validation and volatility-conditioned signal weighting, where coordinated accumulation/distribution patterns amplify momentum when confirmed by microstructure alignment.''}

This parent trajectory focused on identifying \textbf{sustainable momentum} supported by institutional activity, hypothesizing that such momentum is more persistent and reliable.

\subsubsection{Crossover Synthesis}

The LLM synthesized these complementary hypotheses into a unified framework:

\textbf{Offspring Hypothesis}: \textit{``A regime-aware dual-source momentum factor that combines institutional-driven structural momentum (validated by healthy microstructure) and retail-driven speculative momentum (characterized by high attention and deteriorating fundamentals), dynamically weighted by market volatility: amplifying institutional signals in stable regimes and retail reversal signals in turbulent regimes, will generate superior predictive returns.''}

Table~\ref{tab:hypothesis_components} breaks down the hypothesis structure.

\begin{table}[htbp]
\centering
\caption{Hypothesis Component Breakdown}
\label{tab:hypothesis_components}
\small
\begin{tabular}{p{3cm}p{9cm}}
\toprule
\textbf{Component} & \textbf{Description} \\
\midrule
\textbf{Observation} & Parent strategies separately targeting institutional trends and retail herding show moderate predictive power (Rank IC $\sim$0.02--0.025), suggesting combined signals could capture complementary market dynamics. \\
\midrule
\textbf{Justification} & Sustainable price trends require institutional sponsorship and orderly trading, while retail-driven bubbles lack fundamental support and reverse under stress; a hybrid model exploiting both can enhance robustness across market regimes. \\
\midrule
\textbf{Domain Knowledge} & When institutional accumulation coincides with strong price-volume correlation and low volatility, it indicates sustainable momentum; when retail herding in high-attention stocks occurs alongside declining institutional ownership and high volatility, it signals fragile momentum prone to reversal. \\
\bottomrule
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Performance Evaluation}
\label{subsec:performance_evaluation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Table~\ref{tab:factor_performance} presents the backtest results of the evolved factor compared to both parent trajectories and the baseline.

\begin{table}[htbp]
\centering
\caption{Factor Performance Comparison}
\label{tab:factor_performance}
\begin{tabular}{lcccc}
\toprule
\textbf{Metric} & \textbf{Offspring} & \textbf{Parent 1} & \textbf{Parent 2} & \textbf{Baseline} \\
\midrule
IC & 0.0126 & 0.0059 & 0.0069 & 0.0058 \\
Rank IC & \textbf{0.0311} & 0.0216 & 0.0246 & 0.0220 \\
\midrule
ARR (\%) & \textbf{7.80} & --- & --- & 5.20 \\
IR & 0.963 & 1.297 & 1.347 & 0.973 \\
MDD (\%) & $-$11.37 & --- & --- & $-$7.30 \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Performance Analysis}

The crossover operation achieved notable improvements:

\begin{itemize}
    \item \textbf{Predictive Power}: Rank IC improved from 0.0216/0.0246 (parents) to \textbf{0.0311} (offspring), a 26--44\% relative improvement. IC improved by 83--114\% over parents.
    
    \item \textbf{Excess Returns}: Annualized excess return increased from 5.20\% (baseline) to \textbf{7.80\%}, a 50\% improvement.
    
    \item \textbf{Risk Characteristics}: The offspring factor exhibits higher maximum drawdown ($-$11.37\% vs $-$7.30\%), reflecting the more aggressive signal construction. The slightly lower information ratio (0.963 vs 0.973) indicates increased tracking error.
\end{itemize}

\subsubsection{Detailed Backtest Statistics}

Table~\ref{tab:detailed_backtest} provides granular backtest statistics.

\begin{table}[htbp]
\centering
\caption{Detailed Backtest Statistics}
\label{tab:detailed_backtest}
\begin{tabular}{ll|ll}
\toprule
\textbf{Metric} & \textbf{Value} & \textbf{Metric} & \textbf{Value} \\
\midrule
Daily Excess Return (w/o cost) & 0.0328\% & Daily Excess Return (w/ cost) & 0.0128\% \\
Excess Return Std & 0.52\% & Turnover (FFR) & 100\% \\
L2 Train Loss & 0.9936 & L2 Valid Loss & 0.9962 \\
\bottomrule
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{LLM Feedback and Decision}
\label{subsec:feedback_decision}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

After backtesting, the LLM evaluates the results and provides structured feedback to guide subsequent evolution rounds.

\subsubsection{Observations}

The LLM identified the following key observations:
\begin{itemize}
    \item[\checkmark] Higher annualized excess return (7.80\% vs 5.20\% baseline)
    \item[\checkmark] Stronger IC (0.0126 vs 0.0058), indicating improved predictive power
    \item[$\times$] Larger maximum drawdown ($-$11.37\% vs $-$7.30\%)
    \item[$\times$] Slightly lower information ratio (0.963 vs 0.973)
\end{itemize}

\subsubsection{Hypothesis Evaluation}

\textit{``Results partially support the hypothesis. Improved annualized return and IC suggest that combining institutional and retail momentum signals has merit. However, deterioration in risk metrics (higher drawdown, lower information ratio) indicates that without proper regime-adaptive weighting, the combined signals may amplify risks during turbulent periods. The hypothesis likely requires all three components (institutional momentum, retail herding reversal, volatility-adaptive weighting) to work effectively together.''}

\subsubsection{Decision and Recommendations}

\textbf{Decision}: \textsc{Rejected} (for direct deployment)

\textbf{Rationale}: The current factor shows potential but has complexity issues that may lead to overfitting.

\textbf{Recommended Simplification}:
\begin{enumerate}
    \item Use 20-day price-volume correlation as institutional momentum proxy
    \item Use 5-day average intraday returns as retail attention proxy
    \item Weight signals by a simple volatility regime indicator (e.g., ratio of recent to historical volatility)
\end{enumerate}

This feedback demonstrates the iterative refinement process: even when a factor is not immediately accepted, the insights inform subsequent mutation and crossover operations, progressively improving factor quality.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evolution Path Visualization}
\label{subsec:evolution_visualization}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{fig:evolution_path} illustrates the evolution lineage of this factor trajectory.

\begin{figure}[htbp]
\centering
\begin{tikzpicture}[
    node distance=2cm,
    roundbox/.style={rectangle, rounded corners=3pt, draw, minimum width=3.5cm, minimum height=1.2cm, align=center, font=\small},
    arrow/.style={->, thick, >=stealth}
]
    % Parent nodes
    \node[roundbox, fill=purple!10, draw=purple!60] (p1) at (-3.5, 2.5) {
        \textbf{Parent 1}\\
        Round 7 (Mutation)\\
        Rank IC: 0.0216
    };
    \node[roundbox, fill=blue!10, draw=blue!60] (p2) at (3.5, 2.5) {
        \textbf{Parent 2}\\
        Round 6 (Crossover)\\
        Rank IC: 0.0246
    };
    
    % Current node
    \node[roundbox, fill=green!15, draw=green!60, minimum width=4.5cm] (current) at (0, 0) {
        \textbf{Offspring Factor}\\
        Round 8 (Crossover)\\
        Rank IC: \textbf{0.0311}
    };
    
    % Arrows
    \draw[arrow, purple!60, line width=1.5pt] (p1) -- node[midway, left, font=\scriptsize] {Retail Herding} (current);
    \draw[arrow, blue!60, line width=1.5pt] (p2) -- node[midway, right, font=\scriptsize] {Institutional Momentum} (current);
    
    % Improvement annotation
    \node[font=\scriptsize, text=green!60!black] at (0, -1.2) {$\uparrow$ 26--44\% Rank IC improvement over parents};
    
\end{tikzpicture}
\caption{Evolution path diagram showing crossover of two parent trajectories}
\label{fig:evolution_path}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Key Insights from This Case Study}
\label{subsec:case_insights}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This case study demonstrates several key aspects of QuantaAlpha's evolutionary factor mining:

\begin{enumerate}
    \item \textbf{Hypothesis-Driven Crossover}: The LLM synthesizes complementary market hypotheses rather than simply averaging factor expressions, leading to genuinely novel insights.
    
    \item \textbf{Performance Inheritance}: The offspring factor inherits and amplifies the predictive strengths of both parents (26--44\% Rank IC improvement).
    
    \item \textbf{Structured Feedback Loop}: Even rejected factors provide valuable guidance for future iterations, demonstrating the system's ability to learn from both successes and failures.
    
    \item \textbf{Trade-off Awareness}: The LLM explicitly identifies the return-risk trade-off, recommending simplification to improve generalization.
    
    \item \textbf{Interpretability}: Throughout the evolution, factor logic remains interpretable through natural language hypotheses and mathematical formulations.
\end{enumerate}

This iterative process of hypothesis generation, factor construction, backtesting, and feedback enables QuantaAlpha to systematically explore the factor space while maintaining interpretability and avoiding overfitting.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/ablation_table.tex <==
\begin{table}[tb]
  \centering
  \small
\caption{
Ablation study of evolutionary mining components.
}
  \label{tab:ablation_study_two_column}
    \resizebox{\columnwidth}{!}{
  \begin{tabular}{lcccc}
    \toprule
   \multirow{2}{*}{Method} & \multicolumn{4}{c}{Key Metrics} \\
    \cmidrule(lr){2-5}
     &  \multicolumn{1}{l}{\,\,\,\textbf{IC}} &  \multicolumn{1}{l}{\textbf{Rank IC}} &  \multicolumn{1}{l}{\textbf{ARR}} (\%) & \textbf{MDD} (\%) $\downarrow$\\
    \midrule

     \textbf{QuantaAlpha}
& \multicolumn{1}{l}{\textbf{0.0461}}
& \multicolumn{1}{l}{\textbf{0.045}}
& \multicolumn{1}{l}{\textbf{4.53}}
& \multicolumn{1}{l}{\,\,\,\,\textbf{15.1}} \\

     \phantom{Q} -  \emph{w/o} \textbf{Planning}
      & 0.0448\textsuperscript{\textcolor[RGB]{230,180,180}{\tiny -0.0013}}
      & 0.0437\textsuperscript{\textcolor[RGB]{230,180,180}{\tiny -0.0013}}
      & 3.81\textsuperscript{\textcolor[RGB]{180,20,20}{\tiny -0.72}}
      & 16.72\textsuperscript{\textcolor[RGB]{200,50,50}{\tiny +1.62}} \\

     \phantom{Q} -  \emph{w/o} \textbf{Mutation}
      & 0.0382\textsuperscript{\textcolor[RGB]{180,60,60}{\tiny -0.0079}}
      & 0.0371\textsuperscript{\textcolor[RGB]{180,60,60}{\tiny -0.0079}}
      & 3.27\textsuperscript{\textcolor[RGB]{160,20,20}{\tiny -1.26}}
      & 15.58\textsuperscript{\textcolor[RGB]{220,160,160}{\tiny +0.48}} \\

      \phantom{Q} -  \emph{w/o} \textbf{Crossover}
      & 0.0401\textsuperscript{\textcolor[RGB]{220,150,150}{\tiny -0.0060}}
      & 0.0419\textsuperscript{\textcolor[RGB]{220,150,150}{\tiny -0.0031}}
      & 4.02\textsuperscript{\textcolor[RGB]{200,50,50}{\tiny -0.51}}
      & 16.03\textsuperscript{\textcolor[RGB]{220,100,100}{\tiny +0.93}} \\

    \bottomrule
  \end{tabular}
}
\end{table}
